Temporal and Spectral Analysis of 1ES 2344+514 in Two Flaring States Observed by VERITAS

VERITAS observed the bright blazar 1ES 2344+514 during two flaring periods, one from Dec. 17 to Dec. 18, 2015 (MJD 57373-57374) with a peak flux of ~60% of the Crab and another from Nov. 28 to Dec. 3, 2021 (MJD 59546-59551) with a peak flux of ~20% of the Crab. This blazar, located at a redshift of z = 0.044, is classified as an extreme high-frequency-peaked BL Lacertae object (HBL). It is known to be variable, including several previous day-scale flares: Whipple on Dec. 20, 1995, VERITAS on Dec. 7, 2007, and MAGIC on Aug. 11, 2016. The VERITAS near-nightly monitoring of 1ES 2344+514 during the 2015-2016 and 2021-2022 seasons provides good coverage of the pre- and post-flare flux as well as the rise/fall time of the flares. We present the multiwavelength light curves of each flare as well as the very high-energy spectra in the two flare states and the two pre-flare states.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

